Detecting Contextual Anomalies by Discovering Consistent Spatial Regions

We describe a method for modeling spatial context to enable video anomaly detection. The main idea is to discover regions that share similar object-level activities by clustering joint object attributes using Gaussian mixture models. We demonstrate that this straightforward approach, using orders of magnitude fewer parameters than competing models, achieves state-of-the-art performance in the challenging spatial-context-dependent Street Scene dataset. As a side benefit, the high-resolution discovered regions learned by the model also provide explainable normalcy maps for human operators without the need for any pre-trained segmentation model.

==> main_paper.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

%%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% \usepackage[review,algorithms]{wacv}      % To produce the REVIEW version for the algorithms track
%\usepackage[review,applications]{wacv}      % To produce the REVIEW version for the applications track
%\usepackage{wacv}              % To produce the CAMERA-READY version
%\usepackage[pagenumbers]{wacv} % To force page numbers, e.g. for an arXiv version

% Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{times}
% \usepackage{epsfig}


% It is strongly recommended to use hyperref, especially for the review version.
% hyperref with option pagebackref eases the reviewers' job.
% Please disable hyperref *only* if you encounter grave issues, e.g. with the
% file validation for the camera-ready version.
%
% If you comment hyperref and then uncomment it, you should delete
% ReviewTempalte.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).






%%%%%%%%% PAPER ID  - PLEASE UPDATE
\def\wacvPaperID{2699} % *** Enter the WACV Paper ID here
\def\confName{WACV}
\def\confYear{2025}

% Include other packages here, before hyperref.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%% IMPORTANT - These next three lines are CRUCIAL.
%               (1) PLEASE enter your paper ID (given by CMT) replacing the
%                   '****' right below here with the ID from CMT.
%               (2) If you are submitting to the Algorithms track, then uncomment
%                   the \wacvalgorithmstrack line below. If you are submitting to the
%                   Applications track, then uncomment the \wacvapplicationstrack line.
%                   If you do not update this properly, we cannot guarantee
%                   that your paper will be evaluated according to the correct
%                   review criteria!
%               (3) Leave the \wacvfinalcopy commented out for the submission
%                   version, but UNCOMMENT it for your CAMERA-READY upload.
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








% \usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}
% \begin{document}

% %%%%%%%%% TITLE
% \title{Detecting Contextual Anomalies  by Discovering Consistent Spatial Regions}
% %\title{Is it normal? It depends.  }

% \author{Zhengye Yang\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Richard J.~Radke\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \maketitle


%%%%%%%%% ABSTRACT



% \rnote{We need to address that we distill the reason why most newly developed methods can not be applied in StreetScene Dataset: the gap is at the spatial-context. Plus the convolutional autoencoder's innate inferior ability of learning spatial context. We need to mention sometimes the background appearance might be coupled with the spatial context and sometimes not. We need to decouple the background appearance with the spatial normality to ensure a more }
% \begin{figure*}
% \begin{center}
% \includegraphics[width=0.99\linewidth]{figures/semantic_region.png}
% \end{center}
%    \caption{An example of Gaussian Mixture model that learns object-level normalcy distribution within area provided by region discovery in StreetScene dataset. Each learned mixture is a representative normal object-level activity. }
% \label{fig:semantic_explain}
% \end{figure*} 



  


% \rnote{Replace ``Normal'' with Normal/Anomalous (no quotes)}






% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{submitbib}
% % \bibliography{references}
% }

% \end{document}

